Black-Box Approximation and Optimization with Hierarchical Tucker Decomposition

We develop a new method HTBB for the multidimensional black-box approximation and gradient-free optimization, which is based on the low-rank hierarchical Tucker decomposition with the use of the MaxVol indices selection procedure. Numerical experiments for 14 complex model problems demonstrate the robustness of the proposed method for dimensions up to 1000, while it shows significantly more accurate results than classical gradient-free optimization methods, as well as approximation and optimization methods based on the popular tensor train decomposition, which represents a simpler case of a tensor network.

==> helpers.tex <==
% -------
% Helpers
\makeatletter

% \fat - bold font inside the formula or text:
\newcommand{\fat}[1]{\ifmmode\bm{#1}\else\textbf{#1}\fi}

% \set - linear/functional space (R, N, ...):
\newcommand{\set}[1]{\mathbb{#1}}

% \vect - vector:
\newcommand{\vect}[1]{\ensuremath{\fat{#1}}}

% \matr - matrix:
\newcommand{\matr}[1]{#1}

% \tens - tensor (or TT-tensor):
\newcommand{\tens}[1]{\mathcal{#1}}

% \qvect - QTT-vector:
\newcommand{\qvect}[1]{\mathbcal{#1}}

% \qmatr - QTT-matrix:
\newcommand{\qmatr}[1]{\mathcal{#1}}

% \func - function:
\newcommand{\func}[1]{\textsf{#1}}

% \vfunc - vector-function:
\newcommand{\vfunc}[1]{\textsf{\vect{#1}}}

% \ffunc - functional:
\newcommand{\ffunc}[1]{\widehat{#1}}

% \oper - operator:
\newcommand{\oper}[1]{\widehat{#1}}

% \trace - trace of the matrix:
\newcommand{\trace}[1]{\mathrm{Tr}\left( #1 \right)}

% \order - Operator O(...):
\newcommand{\order}[1]{\mathcal{O}\left( #1 \right)}

% \divergence - operator divergence(...):
\newcommand{\divergence}[1]{\mathrm{div}\left[ #1 \right]}

% \der - derivative d * / d *:
\newcommand{\der}[2]{\frac{d \, #1}{d \, #2}}

% \dert - time derivative d * / d t:
\newcommand{\dert}[1]{\der{#1}{t}}

% \derx - spatial derivative d * / d x:
\newcommand{\derx}[1]{\der{#1}{x}}

% \pder - partial derivative d * / d *:
\newcommand{\pder}[2]{\frac{\partial #1}{\partial #2}}

% \pdert - partial time derivative d * / d t:
\newcommand{\pdert}[1]{\pder{#1}{t}}

% \pderx - partial spatial derivative d * / d x:
\newcommand{\pderx}[1]{\pder{#1}{x}}

% \pderxi - partial spatial derivative for i-th component:
\newcommand{\pderxi}[2]{\pder{#1}{\vect{x}_{#2}}}

% \vectorize - vectorization (tensor to vector):
\newcommand{\vectorize}[1]{\fat{vec}\left( #1 \right)}

% \vectl - vector, represented as a list of its elements:
\newcommand{\vectl}[1]{\fat{\left[} #1 \fat{\right]}^{\top}}

% \iflatten - flatten index from multi-index:
\newcommand{\iflatten}[1]{\mathrm{ind}\left( #1 \right)}

% \imulti - multi-index from the flatten index:
\newcommand{\imulti}[1]{\fat{mind}\left( #1 \right)}

% \poi : point (dot) placeholder:
\newcommand{\poi}[0]{\, \cdot \,}

% \note - note (for review):
\newcommand{\note}[1]{ {\color[HTML]{8b1d1d}/* #1 */} }


% ---------
% Shortcuts

\newcommand{\vg}[0]{\vect{g}}            % Vector g
\newcommand{\vi}[0]{\vect{i}}            % Vector i
\newcommand{\vw}[0]{\vect{w}}            % Vector w
\newcommand{\vx}[0]{\vect{x}}            % Vector x
\newcommand{\vy}[0]{\vect{y}}            % Vector y
\newcommand{\vz}[0]{\vect{z}}            % Vector z

\newcommand{\mg}[0]{\matr{G}}            % Matrix g
\newcommand{\mw}[0]{\matr{W}}            % Matrix w
\newcommand{\mx}[0]{\matr{X}}            % Matrix x
\newcommand{\my}[0]{\matr{Y}}            % Matrix y
\newcommand{\mz}[0]{\matr{Z}}            % Matrix z

\newcommand{\tg}[0]{\tens{G}}            % Tensor G
\newcommand{\tw}[0]{\tens{W}}            % Tensor w
\newcommand{\tx}[0]{\tens{X}}            % Tensor x
\newcommand{\ty}[0]{\tens{Y}}            % Tensor y
\newcommand{\tz}[0]{\tens{Z}}            % Tensor z

\newcommand{\ff}[0]{\func{f}}            % Function f
\newcommand{\hff}[0]{\widehat{\ff}}      % Function hat f

\let\div=\relax
\DeclareMathOperator{\div}{div}
\DeclareMathOperator{\vecop}{vec}

\def\ts#1#2{\ensuremath{\tens #1(:,\,#2,\,:)}}
\def\tsi#1#2#3{\ensuremath{\tens{#1_{#3}}(:,\,#2_{#3},\,:)}}


% ---------------
% Helpers (extra)

\newcommand{\method}[1]{\textsf{#1}}
% ------- Gleb --------------------
% -----Letters---------------------
\let\defin=\emph
\def\towidxnot#1#2#3{\ensuremath{{#1}^{(#2)}_{#3}}}
\def\G#1#2{\towidxnot {\tens G}{#1}{#2}}
\def\Kunfold#1{\tens #1^U}
\def\nNch#1#2#3{\towidxnot D{#1+1}{{#2}_{#3}}}
\def\nN#1#2{\towidxnot D{#1}{#2}\gdef\childa{\nNch{#1}{#2}1}\gdef\childb{\nNch{#1}{#2}2}}
\def\nN@glob#1#2{\towidxnot D{#1}{#2}}
\def\nN#1#2{\nN@glob{#1}{#2}\gdef\ch@ldlev{#1}\gdef\ch@ldn@m{#2}\xspace}
\def\child@#1{\nN@glob{\ch@ldlev+1}{{\ch@ldn@m}_#1}\xspace}
\def\childa{\child@1}
\def\childb{\child@2}
\def\nr#1#2{\towidxnot r{#1}{#2}}
\def\nb#1#2{\towidxnot b{#1}{#2}}
%\def\nd#1#2{\towidxnot b{#1}{#2}}
\def\updownstyle{\scriptsize\tt}
\def\nvu#1#2{\ensuremath{v^{\text{\updownstyle up}}_{#1,#2}}\xspace}
\def\niu#1#2{i^{\text{\updownstyle up}}_{#1,#2}\gdef\nvusame{\nvu{#1}{#2}}}
\def\nid#1#2{i^{\text{\updownstyle down}}_{#1,#2}\gdef\nvdsame{\nvd{#1}{#2}}}
\def\nvd#1#2{\ensuremath{v^{\text{\updownstyle down}}_{#1,#2}}\xspace}

\def\dims#1{\ensuremath{\mathbb R^{#1}}}
\DeclareMathOperator{\qr}{QR}
\DeclareMathOperator{\qrp}{QRP}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\maxvol}{MaxVol}
\DeclareMathOperator{\mean}{mean}
\DeclareMathOperator{\std}{std}
\DeclareMathOperator{\setop}{set}

\def\matval#1#2#3{\ensuremath{#1[#2,\,#3]}}

% -----Other-----------------------

\DeclareMathOperator{\joinidx}{joinIDX}
\def\fromoneto#1{\ensuremath{1,\,2,\,\ldots,\,#1}}
\def\fromonetoidx#1#2{\ensuremath{{#1}_1,\,{#1}_2,\,\ldots,\,{#1}_{#2}}}

\def\trans#1{\ensuremath{#1}^{\text{T}}}
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\textit{e.\,g}\onedot} \def\Eg{\textit{E.\,g}\onedot}
\def\ie{\textit{i.\,e}\onedot} \def\Ie{\textit{I.\,e}\onedot}
\def\etc{\textit{etc}\onedot} \def\vs{\textit{vs}\onedot}

\def\comm#1{\textit{// #1}}

\def\red#1{\color{red}#1}
\def\pack#1{\texttt{#1}}

\makeatother

